Robotic Irrigation Water Management: Estimating Soil Moisture Content by Feel and Appearance

In this paper we propose a robotic system for Irrigation Water Management (IWM) in a structured robotic greenhouse environment. A commercially available robotic manipulator is equipped with an RGB-D camera and a soil moisture sensor. The two are used to automate the procedure known as "feel and appearance method", which is a way of monitoring soil moisture to determine when to irrigate and how much water to apply. We develop a compliant force control framework that enables the robot to insert the soil moisture sensor in the sensitive plant root zone of the soil, without harming the plant. RGB-D camera is used to roughly estimate the soil surface, in order to plan the soil sampling approach. Used together with the developed adaptive force control algorithm, the camera enables the robot to sample the soil without knowing the exact soil stiffness a priori. Finally, we postulate a deep learning based approach to utilize the camera to visually assess the soil health and moisture content.

==> thesis-texts/car-imp.tex <==

\section{Position-based impedance control}


One common, widely recognized and practical method for compliant control of position based robots is the position-based impedance control. This concept allows simultaneous control of manipulator position and contact force, while only a single interface is available at low joint level control, such as joint position control. It should be noted that impedance control can be implemented in Cartesian space, when the aim is to control the end-effector interaction with the environment, but it can be implemented at joint level as well, when safety if the primary concern. The use case described in this work deals with the former application, namely Cartesian impedance.  %The Position-based impedance control has been widely recognized as a practical approach for compliant control of industrial robots contacting the environment.

The objective of the basic impedance controller is to establish a desired user-specified dynamic relationship between contact force and robot position, referred to as the \textit{target impedance}. %The basic impedance control concept is to establish a desired user-specified dynamical relationship between contact force and position, referred to as the \textit{target impedance}. 
This work is built upon the structure of a basic position-based impedance control loop, shown in Fig. \ref{fig:impedance_control_scheme}. The standard elements of the aerial manipulator control scheme, namely position and attitude controllers, are extended with an impedance filter. The impedance filter determines a position setpoint for the position controller, based on the desired contact force during the physical interaction. The inner loop represents the non-modified robot position controller. Since there is no direct force control interface for the robot, the outer loop uses force feedback signal by modifying the inputs to the position controller, at the same time satisfying the impedance filter dynamic equation. To model the robot-environment interaction, the environment is considered as an equivalent linear spring, with $n \times n$ constant diagonal stiffness $K_e$. This way, the measured contact force can be considered a result of a linear spring compression, or simply
\begin{equation}
\label{eq:force_meas}
\textbf{F} = K_e (\textbf{X} - \textbf{X}_e),
\end{equation}
where $\textbf{F}$ is an $ n \times 1$ vector that represents the measured force, $\textbf{X}$ is an $ n \times 1$ measured robot position vector, and $\textbf{X}_e$ is the position vector of the environment, with dimensions $ n \times 1$. The environment position $\textbf{X}_e$ is considered constant in the unexcited state, namely in the state without contact. As the (measured) robot position $\textbf{X}$ progresses into the environment, there is a displacement between the measured robot position and the unexcited environment position, i.e. the elasticity of the environment generates a force that acts on the robot. 

The impedance filter defines the target impedance behaviour of the robot-environment interaction system. The filter is designed as a linear second-order system. This enables setting the dynamic relationship between the robot position and the force tracking error $\textbf{E} = \textbf{F}_r - \textbf{F}$, so that it mimics a mass-spring-damper system. The $ n \times 1$ force reference vector $\textbf{F}_r$ can be freely chosen by the user. Throughout this work, the target impedance is defined as
\begin{equation}
\label{eq:targetImpedance}
\textbf{E} = M (\ddot{\textbf{X}}_c - \ddot{\textbf{X}}_r) + B (\dot{\textbf{X}}_c - \dot{\textbf{X}}_r) + K (\textbf{X}_c - \textbf{X}_r),
\end{equation}
where $M$, $B$ and $K$ are the $n \times n$ constant diagonal mass, damping and stiffness matrices of the target impedance, respectively. These matrices are arbitrarily specified by user, setting the system behaviour to the desired target impedance. Signals $\textbf{X}_c$ and $\textbf{X}_r$ are vectors in Cartesian space, and represent the commanded and reference position of the robot, respectively. The commanded position is the one used as input to the robot inner loop position controller, usually through an inverse kinematics or Jacobian in the form of joint position. The reference position, on the other hand, is the user defined desired cartesian position of the robot. 

During free-space motion, while there is no force tracking error $\textbf{E} = \textbf{0}$, the commanded position $\textbf{X}_c$ tracks the reference position $\textbf{X}_r$ accurately, with the dynamics specified with Equation \eqref{eq:targetImpedance}. As the end-effector comes into contact with the environment, the contact force $\textbf{F}$ is measured by the force sensor. This results in a modified robot position command $\textbf{X}_c$, since at that point, the dynamics of the target impedance cannot allow precise tracking of referenced position  $\textbf{X}_r$, without resulting in force tracking error signal  $\textbf{E}$. In other words, the impedance filter balances the position and force tracking error, depending on the filter parameters. A more detailed position-based impedance control analysis can be found in \cite{Seraji1993}.

\begin{figure}[h!]
\centering
\includegraphics[width=\columnwidth]{images/impedance/impedance_control_sema.pdf}
\caption{Position-based impedance control scheme. The impedance filter output is reference for the UAV position controller, hence position-based impedance control.}
\label{fig:impedance_control_scheme}
\end{figure}

Consider the practical case, in which the environment stiffness $K_e$ is unknown, and the exact position of the environment $\textbf{X}_e$ is inaccurate. While in contact with the environment, these uncertainties can considerably degrade the performance of the system. To analyze this behavior, we start from the linear spring model of the environment, with stiffness $K_e$. For simplicity, we consider a case where force is applied along one axis only, with equivalent stiffness $k_e$. As already stated in Eq. \eqref{eq:force_meas}, the measured force can be considered a result of spring compression, namely $f(t) = k_e (x(t) - x_e(t))$. Let us expand the force error $e(t)$ as
\begin{equation}
\label{eq:forceError}
e(t) = f_r(t) - f(t) = f_r(t) - k_e (x(t) - x_e(t)).
\end{equation}
From the force tracking error equation \eqref{eq:forceError}, the position of the aerial manipulator can be expressed as:
\begin{equation} \label{eq:pos_man}
	x (t) = \frac{f_r  (t) - e (t)}{k_e} + x_e (t).
\end{equation}
Assuming further that the force reference $f_r(t)$ is constant, $f_r(t) = F_r$, the time derivatives of Eq. \eqref{eq:pos_man} yield:
\begin{align}
    \label{eq:pos_man_d}
    \dot{x}(t) = \frac{\dot{e}(t)}{k_e} + \dot{x_e}(t) \\
    \label{eq:pos_man_dd}
    \ddot{x}(t) = \frac{\ddot{e}(t)}{k_e} + \ddot{x_e}(t)
\end{align}
Assuming that the aerial manipulator tracks the position reference with negligible dynamics, $x(t) \approx x_c(t)$, the force tracking error dynamics can be derived from the Equation \eqref{eq:pos_man}, Equation \eqref{eq:pos_man_d}, Equation \eqref{eq:pos_man_dd} and the target impedance Equation \eqref{eq:targetImpedance}:
\begin{align}
\label{eq:forceErrorDynamics}
\begin{split}
m\ddot{e}(t)+b\dot{e}(t)+(k +k_e)e(t) = &m(\ddot{x_e}(t) - \ddot{x_r}(t))\\
&+b(\dot{x_e}(t) - \dot{x_r}(t)) \\
&+k(F_r + k_e x_e(t) - k_e x_r(t).
\end{split}
\end{align}
Here, the target impedance behaviour is also defined along one axis only, with mass, damping and stiffness parameters $m$, $b$, and $k$ respectively. The Equation \ref{eq:forceErrorDynamics} shows that it is possible to control the force error trajectory through the  input signal $x_r$. The steady-state force error $e_{ss}$ can then be obtained by applying the final value theorem to the Laplace transform of Equation \eqref{eq:forceErrorDynamics}:
\begin{equation}
e_{ss} = \frac{k}{k+k_e}[(F_r +k_e x_e)-k_e x_r].
\end{equation}
The steady-state force error will be zero, if the following condition on the reference position trajectory is satisfied:
\begin{equation}
\label{eq:pos_ss}
x_r = \frac{F_r}{k_e} + x_e.
\end{equation}
In other words, if the precise environment position $x_e$ is known, as well as the value of the environment equivalent stiffness $k_e$, a reference position trajectory $x_r$ can be generated, that will result in robot-environment interaction in which exactly the desired contact force is exerted. However, the environmental parameters are in practice never known precisely, and even small errors in the environment parameters $k_e$ and $x_e$ can result in large force errors. One possible solution to this issue is the estimation of these parameters. As we show in the following chapter, the estimation of these parameters can be used in adaptation of the impedance filter inputs, resulting in desired robot behaviour and precise position and contact force tracking, even with environment position and stiffness unknown a-priori.
\clearpage

\section{Adaptive impedance control}
\todo[inline]{prepraviti opisati da je ideja da se uzme ovaj gore adaptacijski zakon i da se mijenja samo krutost a da poziciju kao znamo u naprijed}
\label{sec:AdaptiveImpedanceControl}

The method we propose here is developed for deployment in robot-environment interaction tasks in which the working environment is not completely known. In particular, we assume a robot manipulation setup in which the environment stiffness is unknown, but the position of the environment can be obtained through other remote sensing setup, such as visual or radar/lidar based sensing. 

\begin{equation}
\label{eq:adaptiveControlLaw}
z_r(t) = g(t) + k_p(t)e(t) + k_d(t)\dot{e}(t),
\end{equation}
where $k_p(t)$ and $k_d(t)$ are the adaptive, proportional and derivative gains while $g(t)$ is the auxiliary signal which compensates for the steady-state error. Direct adaptive impedance control scheme is shown in Figure \ref{fig:adaptive_impedance_control_scheme}.

\begin{figure}[h!]
\centering
\includegraphics[width=\columnwidth]{images/impedance/adaptive_impedance_control_sema.pdf}
\caption{Adaptive impedance control scheme.}
\label{fig:adaptive_impedance_control_scheme}
\end{figure}

\subsection{Derivation of the Adaptation Laws}
\label{AdaptationLaws}
The derivation of the adaptation laws requires an assumption that the variation of the system parameters is slower than the speed of adaptation. If this assumption is not satisfied, the adaptive gains will not converge. Therefore, we use proportional-plus-integral adaptation laws derived using an improved Lyapunov-based adaptation method for decentralized systems. These laws, in comparison to the conventional integral laws, have better transient response, improved convergence and increased flexibility \cite{Seraji1989}.

The adaptation law is derived starting from Equation \eqref{eq:pos_ss}. An adaptive parameter $\kappa(t)$ is introduced, that can account for elastic properties of environment under external force, by adapting the position reference with respect to initial position of the environment and force reference:
\begin{equation} 
\label{eqn:pos_kappa}
	x_r (t) =  \kappa (t) F_r + x_e (t).
\end{equation}
Assuming that force reference $F_r$ is constant, the time derivatives of Equation \eqref{eqn:pos_kappa} are:
\begin{align} 
\label{eqn:pos_kappa_dot}
\dot{x_r} (t) =  \dot{\kappa} (t) F_r + \dot{x_e} (t), \\
\label{eqn:pos_kappa_ddot}
\ddot{x_r} (t) =  \ddot{\kappa} (t) F_r + \ddot{x_e} (t),
\end{align}
We first assume that the environment position $x_e(t)$ is precisely known and that only environment stiffness needs to be adapted. This can be ensured e.g. by an auxiliary sensory system based on visual or other non-contact technology. To derive the adaptation laws for $\kappa (t)$, we first substitute $x_r(t)$, $\dot{x_r} (t)$ and $\ddot{x_r} (t)$ in the equation of the force error dynamics \eqref{eq:forceErrorDynamics} with \eqref{eqn:pos_kappa}, \eqref{eqn:pos_kappa_dot} and \eqref{eqn:pos_kappa_ddot}. From here, we derive the equation for the complete adjustable system:
\begin{equation}
\label{eq:adjustableSystemCompact}
\ddot{e}(t) + \phi_1(t)\dot{e}(t) + \phi_2(t)e(t) = \phi_3(t),
\end{equation}
where
\begin{align}
\label{eq:a1a2a3gains}
 a_1(t) &= \frac{b}{m}, \nonumber \\
 a_2(t) &= \frac{k + k_e)}{m}, \nonumber \\
 \phi_1(t) &= F_r [ \frac{k (1 - k_e \kappa (t)) - b k_e \dot{\kappa} (t)}{m} - k_e \ddot{\kappa} (t)].
\end{align}
Writing $\textbf{e} = [e(t), \dot{e}(t)]^\top$, the state-space representation of Equation \eqref{eq:adjustableSystemCompact} can be expressed as 
\begin{equation}
\label{eq:statespaceError}
\dot{\textbf{e}} =	\begin{bmatrix}
						0			& 1 \\
						-a_2(t) 	& -a_1(t)
					\end{bmatrix} \textbf{e} +
					\begin{bmatrix}
						0 \\
						\phi_1(t)
					\end{bmatrix},
\end{equation}
\todo[inline]{provjeriti stabilnost s hurwitzom}
We can write Equation \eqref{eq:statespaceError} as:
\begin{equation}
\label{eq:trackingErrorEq}
\dot{\textbf{e}} = D\textbf{e} + \textbf{h},
\end{equation}
where
\begin{align}
\label{eq:matrixD}
D &= \begin{bmatrix}
    0			& 1 \\
	-a_2(t) 	& -a_1(t)
    \end{bmatrix}, \\
\label{eq:matrixh}
\textbf{h}(t) &= \begin{bmatrix}
                0 \\
				\phi_1(t)
             \end{bmatrix}.
\end{align}
Since error dynamic is stable, Equation \eqref{eq:adjustableSystemCompact}, for all $Q = Q^\top \in \mathbb{R}^{2x2}$ there exists a unique positive-definite matrix $P = P^\top \in \mathbb{R}^{2x2}$ satisfying the Lyapunov equation
\begin{equation}
\label{eq:lyapunovEquation}
D^\top P + P D = - Q.
\end{equation}
Choosing $Q$ as
\begin{equation}
Q = \begin{bmatrix}
	2q_1  & 0 \\
	0	  & 2q_2
	\end{bmatrix},
\end{equation}
where $q_1$ and $q_2$ are positive scalars. From Equation \eqref{eq:lyapunovEquation}, we can derive the solution for $P$:
\begin{equation}
P = \begin{bmatrix}
	p_1 & p_2 \\
	p_2 & p_3
	\end{bmatrix} =
	\begin{bmatrix}
	\frac{1}{a_1} (q_1 (1+\frac{a_1^2}{a_2}) + a_2 q_2) & \frac{q_1}{a_2} \\
	\frac{q_1}{a_2} & \frac{1}{a_1} (\frac{q_1}{\a_2} + q_2)
	\end{bmatrix}.
\end{equation}
Elements of matrix $P$ must be chosen as $p_1,p_2,p_3 > 0$ and $p_2 < p_3 \frac{b}{m}$ for the matrices $Q$ and $P$ to be positive-definite.

The adaptation law determines the dynamics of the adaptation parameter $\kappa (t)$ and defines the dynamics of the contact force error. Formally, the adaptation law should enforce $\phi_1(t) \xrightarrow{} \phi_1^*$ such that $e(t) \xrightarrow{} 0$ and $\kappa (t) \xrightarrow{} 1/k_e$. To derive the adaptation laws, we can define the following positive-definite scalar Lyapunov function candidate:
\begin{align}
\label{eq:lyapunovFunctionCandidate}
V(\textbf{e},\Phi) = \textbf{e}^\top P \textbf{e} + (\Phi -\Phi^*)^\top \Gamma^{-1} (\Phi -\Phi^*),
\end{align}
where $\Gamma = [\gamma_1]$, $\gamma_1$ is positive constants, $\Phi = [ \phi_1(t) ]$ is parameter vector,  $P$ is matrix that satisfies the Lyapunov equation \eqref{eq:lyapunovEquation} and $\Phi^* = [ \phi_1^*(t) ]$. The time derivative of \eqref{eq:lyapunovFunctionCandidate} is given with
\begin{align}
\label{eq:dlyapunovFunctionCandidate}
\dot{V}(\textbf{e},\Phi) = &-\textbf{e}^\top Q \textbf{e} + 2 \textbf{e}^\top P \textbf{h}(t) \nonumber\\
&+ (\dot{\Phi} -\dot{\Phi}^*)^\top \Gamma^{-1} (\Phi -\Phi^*) \nonumber\\
&+ (\Phi -\Phi^*)^\top \Gamma^{-1} (\dot{\Phi} -\dot{\Phi}^*).
\end{align}
Further simplifying the equations, the time derivative of $V$ can be written as
\begin{align}
\dot{V}(\textbf{e},\Phi) = &-\textbf{e}^\top Q \textbf{e} \nonumber\\
&+ \frac{2}{\gamma_1}\phi_1(t)(\dot{\phi}_1(t)-\dot{\phi}_{1}^{*}(t)) + 2q(t)\phi_1(t) \nonumber \\
&- \frac{2}{\gamma_1} \phi_{1}^{*}(t)(\dot{\phi}_1(t)-\dot{\phi}_{1}^{*}(t)),
\end{align}
where $q(t) = p_2 e(t) + p_3 \dot{e}(t)$. To ensure asymptotic stability, the time derivative of $V$ must be a negative-definite function. In that case, we set
\begin{align}
\label{eq:phiphi}
\frac{2}{\gamma_1}\phi_1(t)(\dot{\phi}_1(t)-\dot{\phi}_{1}^{*}(t)) - 2q(t)\phi_1(t) = 0 \nonumber \\
\Rightarrow \dot{\phi}_1(t)-\dot{\phi}_{1}^{*}(t) = -\gamma_1 q(t).
\end{align}
The Equation \eqref{eq:dlyapunovFunctionCandidate} is reduced to 
\begin{align}
\dot{V}(\textbf{e},\Phi) = &-\textbf{e}^\top Q \textbf{e} + 2 \phi_{1}^{*}(t) q(t).
\end{align}
Now, let us choose $\phi_{1}^{*}(t)$ as follows:
\begin{align}
\label{eq:phi}
\phi_{1}^{*}(t) &= -\gamma_{1}^{*}q(t),
\end{align}
where $\gamma_{1}^{*}$ is zero or positive constant. Hence, Equation \eqref{eq:dlyapunovFunctionCandidate} reduces to
\begin{align}
\label{eq:lyapunovSimplifiesEq}
\dot{V}(\textbf{e},\Phi) = &-\textbf{e}^\top Q \textbf{e} - 2\gamma_{1}^{*}q(t)^2,
\end{align}
which is a negative-definite function of $\textbf{e}$. According to the Lyapunov stability theorem, the expression Equation \eqref{eq:lyapunovSimplifiesEq} guarantees the global stability and the global tracking convergence of the system using the control law \eqref{eq:adaptiveControlLaw}. From equalization of \eqref{eq:phiphi} and \eqref{eq:phi}, the adaptation law for $\Phi$ can be obtained
\begin{equation}
\label{eq:phiAdaptationLaws}
\dot{\Phi} = \begin{bmatrix}
			-\gamma_1 q(t) - \gamma_{1}^* \dot{q}(t)
			\end{bmatrix}.
\end{equation}
The adaptive gains $\kappa$ defined in the control law \eqref{eq:adaptiveControlLaw} can be derived from \eqref{eq:phiAdaptationLaws} and \eqref{eq:a1a2a3gains}:
\begin{equation}
\label{eq:finalphi}
\dot{\Phi} = \begin{bmatrix}
			\dot{\phi}_1
			\end{bmatrix} =
			\begin{bmatrix}
			-F_r (\frac{k k_e \dot{\kappa}(t) + b k_e \ddot{\kappa}(t)}{m} + k_e \dddot{\kappa}(t))
			\end{bmatrix}.
\end{equation}
The adaptation law is finally obtained by taking the Equation \eqref{eq:phiAdaptationLaws}, and substituting $\dot{\phi}(t)$ with Equation \eqref{eq:finalphi}:
\begin{align}
k \dot{\kappa} (t) + b \ddot{\kappa} (t) + m \dddot{\kappa} (t) &= - \gamma_1 q (t) + \gamma_{1}^* \dot q (t), \nonumber \\
q(t) &= p_2 e(t) + p_3\dot{e}(t).
\end{align}


==> thesis-texts/mars-imp.tex <==


\subsection{Impedance control}

Compliant behaviour can be attained with position based robots, with additional sensors and a compliant control framework. One common approach relies on position based impedance control, often called admittance control. This control concept relies on a multiple input filter that allows simultaneous control of both position, and contact forces, through the same control interface on the joint level. Namely, the position control interface of the robot is referenced with an input calculated taking into account the force feedback signal as well, by satisfying the impedance filter dynamic equation. In this work, impedant behaviour is analysed in the Cartesian space, for manipulation and interaction of the robot end-effector with the environment. Similar concept exists at the joint level, where joint position impedant control can be implemented for each joint. In this case, local joint torques are needed, which is rarely available with classical industrial manipulators. This approach is therefore usually only possible with collaborative robots.

The Cartesian impedance controller is tuned to achieve a desired dynamic behavior of the robot in interaction with the environment. During this interaction the environment is most commonly considered as a linear spring, and described with a linear approximation as in eq. \ref{eq:force_meas}: 
\begin{equation}
\label{eq:force_meas}
\textbf{F} = K_e (\textbf{X} - \textbf{X}_e),
\end{equation}
where $\textbf{X}$ is an $ n \times 1$ measured robot position vector, and $\textbf{X}_e  \in n \times 1$ is the position vector of the environment in an unexcited state. With the linear spring approximation, the environment is described with a constant diagonal stiffness matrix $K_e \in n \times n$. $\textbf{F} \in n \times 1$ then represents the force generated by the compressed environment along all axes of interest, in case the robot end effector penetrates into the environment. The displacement between the measured robot position and the unexcited environment position, i.e. the elasticity of the environment generates a force that acts on the robot. In other words, $\textbf{F}$ is the measured contact force, as a result of the linear spring compression.

The impedance filter enables describing the entire robot-environment interaction system with an equivalent spring as well. By defining the target impedance behavior of the system, the second order linear system can be designed that enables setting the dynamic relationship between the robot position and the force tracking error $\textbf{E} = \textbf{F}_r - \textbf{F}$, so that it mimics a mass-spring-damper system. The $ n \times 1$ force reference vector $\textbf{F}_r$ can be freely chosen by the user. The target impedance is given with
\begin{equation}
\label{eq:targetImpedance}
\textbf{E} = M (\ddot{\textbf{X}}_c - \ddot{\textbf{X}}_r) + B (\dot{\textbf{X}}_c - \dot{\textbf{X}}_r) + K (\textbf{X}_c - \textbf{X}_r),
\end{equation}
where $M$, $B$ and $K$ are the $n \times n$ mass, damping and stiffness matrices of the target impedance, respectively. These matrices, most often constant and diagonal, enable setting the desired target impedance to the system by arbitrary specifying the matrix elements. The signals $\textbf{X}_c$ and $\textbf{X}_r$ are Cartesian vectors representing the commanded and reference position of the robot, respectively. The reference position is the one provided by the user, or by a higher level controller. The commanded position, on the other hand, is the reference used as input for the robot lower level Cartesian position control, or often, using inverse kinematics or Jacobian, directly at a joint level position control. 

The behavior of the impedance filter enables smooth control of the robot both in contact with the environment, and during free-space motion. In this case, when there is no measured contact force and the reference is zero, there is no force tracking error $\textbf{E} = \textbf{0}$. The commanded position $\textbf{X}_c$ then tracks the reference position $\textbf{X}_r$ accurately, filtered through the dynamics specified with \eqref{eq:targetImpedance}. On the other hand, when the robot comes into contact with the environment, the force sensors measure some contact force $\textbf{F}$. This affects the robot position command $\textbf{X}_c$, and, with a constant reference position $\textbf{X}_r$, the position tracking cannot be accurate any longer. In other words, the impedance filter aims to balance between the position and force tracking errors, depending on the desired behavior, specified through the filter parameters. 

